From Traditional to Modern : Domain Adaptation for Action Classification in Short Social Video Clips

Short internet video clips like vines present a significantly wild distribution compared to traditional video datasets. In this paper, we focus on the problem of unsupervised action classification in wild vines using traditional labeled datasets. To this end, we use a data augmentation based simple domain adaptation strategy. We utilise semantic word2vec space as a common subspace to embed video features from both, labeled source domain and unlablled target domain. Our method incrementally augments the labeled source with target samples and iteratively modifies the embedding function to bring the source and target distributions together. Additionally, we utilise a multi-modal representation that incorporates noisy semantic information available in form of hash-tags. We show the effectiveness of this simple adaptation technique on a test set of vines and achieve notable improvements in performance.

==> src/relatedwork.tex <==
\section{Background and Related Work}
\label{sec:relwork}
Videos on the web provide a rich source for training generalized classifiers, however 
manual labeling of web-data is non-trivially expensive. Categorizing such data directly 
using traditionally trained systems has many limitations owing to dataset bias intrinsic to the collection 
process and domain differences. \citet{YouTubeCat} use hierarchical category taxonomy tree, designed by professional linguists, to categorize 
Youtube videos. However, this approach cannot be extended for action classification as it is difficult to hand-craft a generalized 
taxonomy for actions. Approaches that particularly handle action classification in web-videos loosely fall under the following 
three categories. 

\paragraph{Complex Datasets:} Early approaches in action recognition focused on curating increasingly complex and wilder video 
distributions for training classifiers that would work on real-world data \cite{ActionsAsSpaceTimeShapes_pami07, Kuehne11, 
, UCF101, 2015trecvidover}. Refer to \cite{Chaquet:2013:SVD:2459519.2459780} for a comprehensive survey of action classification 
datasets. However, no distribution is generalized enough to fully capture the real-world data. 

\paragraph{Complex Features:} Many approaches focus on improving the feature representation by incorporating 
spatio-temporal constructs \cite{ActionsAsSpaceTimeShapes_pami07, spatioTemporalwords, Weinland:2006:FVA:1225844.1225855}, 
appropriate human body modeling \cite{Ikizler20091515, Jhuang:ICCV:2013}, extending successful 
image features to videos \cite{Scovanner:2007:SDA:1291233.1291311, Klaser_aspatio-temporal, actionlets}. For a complete 
reference see survey papers \cite{survey1} and \cite{survey2}). Recently, increasingly complex features from large-scale dictionaries and 
Convolutional Neural Networks (CNN) are becoming popular. Again, these features are only meaningful with large 
generalized annotated datasets and resource intensive supervised training.

In our method we deal with a complex but unlabeled dataset. We use traditional labeled dataset and
present a simple incremental approach to transfer knowledge from this simpler labeled source dataset 
to a wilder unlabeled target dataset. The class of methods that try to mitigate the bias/shift between source and 
target dataset fall under the category of \textit{transfer learning} methods. Recently, many methods are 
proposed that focus on dataset bias shift\cite{EfrosBias,datasetIssues}, domain adaptation \cite{adaptiveDict,whatYouSeeDomain}, 
zero-shot learning \cite{zslearn}, heterogeneous/multi-modal transfer \cite{NIPS2008_3550} and other transfer learning methods 
\cite{daumeiii,GFK,YangDA,5288526} etc. Such methods have shown promise in building more generalizable systems. 
However, most of these methods work on image/object category problems or text-data problems and their application to 
web-scale wild video distributions remain untested. 

\citet{SultaniBias} propose a feature encoding that accounts for the bias 
introduced by dataset specific backgrounds for video classification. However, this method requires both 
source and target videos to be labeled. Our target set is unlabeled and has no separate training phase. 
Hence our method is unsupervised and transductive. 

A recent related work \cite{NIPS2008_3550} uses sparse dictionary constraints to improve zero-shot learning (ZSL) 
performance. This assumes disjoint source and target labels and restricts embedding function to be a linear transformation. 
Similary \cite{7350760} uses regressors and data augmentation to improve ZSL performance.
Our method differs from theirs due to its incremental relearning of neural network which allows more non-linearity 
in the embedding function and does not enforce the disjoint assumption. Also, we report results on much wilder 
and challenging dataset of vines and also utilize multi-modal information in the form of tags to improve performance.
  

% In recent years, increasingly complex and 
% challenging datasets are introduced to remedy this problem. 
% Some popular datasets for action classification are UCF101 \cite{UCF101}, 
% HMDB \cite{Kuehne11}, Weizmann dataset \cite{ActionsAsSpaceTimeShapes_pami07}, 
% TRECVID \cite{2015trecvidover},etc. For a comprehensive list, we recommend  
% survey paper by \citet{Chaquet:2013:SVD:2459519.2459780}.

% %In order to capture real world scenarios such datasets are becoming more and more challenging. 
% 
% Despite several best efforts to create generalized datasets, most datasets present distribution 
% specific bias as capture bias, selection bias, negative set bias etc. 
% Hence, classifiers trained on one dataset fail to achieve comparable performance 
% on another dataset. This was well 
% demonstrated in the case of object recognition by \cite{EfrosBias,datasetIssues}. 
% This observation has inspired the research community to explore better transfer 
% learning techniques wherein learning is transferred between domains
% based on rules derived from prior information, noisy labels, 
% weak supervision or unsupervised associations. A few well known transfer learning methods
% use feature augmentation \cite{daumeiii}, cross-domain dictionary/basis 
% learning \cite{adaptiveDict,GFK}, feature-space transformation \cite{whatYouSeeDomain} 
% or adaptive classification strategies \cite{YangDA,YouTubeCat}.
% 
% 
% 
% \citet{genericAnnotation} use semi-supervised learning for 
% \textit{event} detection and localization in web videos using a graph based 
% approach. They use close-captions, scripts, subtitles and web-casting text 
% to build an expert-labeled training dataset. 
% Similarly \citet{scriptBasedAction} 
% % focus on human action recognition and
% use movie scripts as weak annotations which are 
% unavailable in case of vines. 
% \cite{nearDuplicates, webBasedPose} 
% rely on web search and visual similarity between frames for tag propagation. 
% We base our method on more robust motion features (dense trajectories) instead of 
% only temporally extended shape similarity features (keypoints and SIFTs). 
% \citet{DuanWebData} use weak web labels to assist their \textit{event detection} classifiers on higher quality consumer
%video collections. Our approach instead is to use well annotated datasets like UCF to learn classifiers on noisy web domain.
% \citet{SultaniBias} compute 
% separate background and foreground features and define pixel weights to improve human action performance across datasets. 
% Their approach is novel
% but they do not leverage multi-modal data in their system. Additionally we exploit semantic 
% relations by learning an embedding function for the two modalities being used.
% 
% % Keeping in line with the previous works we call our assisting source domain (UCF videos) as \textit{auxiliary domain} 
% and the web videos (vines) constitute \textit{target domain}. We build a confidence score by embedding video features 
% and tags in a common semantic space. This is a well known method for combining multi-modal data. 
% But in addition to this we also update our embedding function as our source distribution is iteratively updated.
% We show that this favourably changes our source distribution (which is initially only auxiliary domain) to 
% target distribution (which is composed of mixture of both auxiliary and target domains).

